A Systematic Investigation of KB-Text Embedding Alignment at Scale

Knowledge bases (KBs) and text often contain complementary knowledge: KBs store structured knowledge that can support long range reasoning, while text stores more comprehensive and timely knowledge in an unstructured way. Separately embedding the individual knowledge sources into vector spaces has demonstrated tremendous successes in encoding the respective knowledge, but how to jointly embed and reason with both knowledge sources to fully leverage the complementary information is still largely an open problem. We conduct a large-scale, systematic investigation of aligning KB and text embeddings for joint reasoning. We set up a novel evaluation framework with two evaluation tasks, few-shot link prediction and analogical reasoning, and evaluate an array of KB-text embedding alignment methods. We also demonstrate how such alignment can infuse textual information into KB embeddings for more accurate link prediction on emerging entities and events, using COVID-19 as a case study.

==> todonotes.tex <==
%%%% TODONOTE MACROS
\usepackage[disable]{todonotes}
% \usepackage{todonotes}
\makeatletter
\newcommand*\iftodonotes{\if@todonotes@disabled\expandafter\@secondoftwo\else\expandafter\@firstoftwo\fi}  % defines \iftodonotes{<true>}{<false>}, thanks to https://tex.stackexchange.com/questions/126559/conditional-based-on-packageoption
\makeatother
\newcommand{\noindentaftertodo}{\iftodonotes{\noindent}{}\ignorespaces}
% Note that these macros accept optional arguments such as size=\small, bordercolor=red, and so on.  
\newcommand{\fixme}[2][]{{\todo[color=yellow,size=\scriptsize,fancyline,caption={},#1]{#2}}} % to mark stuff that you know is missing or wrong when you write the text
\newcommand{\note}[4][]{{\todo[author=#2,color=#3,size=\scriptsize,fancyline,caption={},#1]{#4}}} % default note settings, used by macros below.

% For commenters who do not want to define their own macro:
% Specify author name in first required argument.
\newcommand{\notewho}[3][]{\note[#1]{#2}{blue!40}{#3}}
\newcommand{\ysu}[2][]{\note[#1]{ysu}{cyan!40}{#2}}
\newcommand{\wchen}[2][]{\note[#1]{wchen}{cyan!40}{#2}}
\newcommand{\vardaan}[2][]{\note[#1]{vardaan}{cyan!40}{#2}}

% Capitalized versions are inline paragraphs instead of margin notes.
\newcommand{\Fixme}[2][]{\fixme[inline,#1]{#2}\noindentaftertodo}
\newcommand{\Notewho}[3][]{\notewho[inline,#1]{#2}{#3}\noindentaftertodo}
\newcommand{\Ysu}[2][]{\ysu[inline,#1]{#2}\noindentaftertodo}

% Insert response within a todo note.
\newcommand{\response}[1]{\vspace{3pt}\hrule\vspace{3pt}\textbf{#1: }}
% If todonotes is turned on, expand the page width to allow for wider margin notes.
\newlength{\extramargin}
\setlength{\extramargin}{60mm}  % user-tunable
\usepackage{calc}
\iftodonotes{\usepackage[paperwidth=\paperwidth+\extramargin*2,marginparwidth=\marginparwidth+\extramargin,width=\textwidth,height=\textheight]{geometry}}{}
%%%% end todonote macros
